Image Classification with Consistent Supporting Evidence

Adoption of machine learning models in healthcare requires end users' trust in the system. Models that provide additional supportive evidence for their predictions promise to facilitate adoption. We define consistent evidence to be both compatible and sufficient with respect to model predictions. We propose measures of model inconsistency and regularizers that promote more consistent evidence. We demonstrate our ideas in the context of edema severity grading from chest radiographs. We demonstrate empirically that consistent models provide competitive performance while supporting interpretation.

==> figures.tex <==

\begin{figure}[htbp]
    \floatconts
        {fig:consistent_tikz_example}
        {\caption{
            A graphical illustration of a case where evidence are consistent. We have grouped evidence $\sI(y)$ into supernodes. A gray node indicate existence of a positive label.
        }}
        {
    \begin{center}
    \begin{tikzpicture}
        \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=1cm] (e0) at (-3,0)   { $\sI(0)$ };
        \node [circle,draw=black,fill=gray!20,inner sep=0pt,minimum size=1cm] (e1) at (-1,0) { $\sI(1)$ };
        \node [circle,draw=black,fill=gray!20,inner sep=0pt,minimum size=1cm] (e2) at ( 1,0) { $\sI(2)$ };
        \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=1cm] (e3) at (3, 0)   { $\sI(3)$ };
        \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=1cm] (y0) at (-3,1.6) { $0$ };
        \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=1cm] (y1) at (-1,1.6) { $1$ };
        \node [circle,draw=black,fill=gray!20,inner sep=0pt,minimum size=1cm] (y2) at ( 1,1.6) { $2$ };
        \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=1cm] (y3) at (3, 1.6) { $3$ };
    
        \path [draw,->] (y0) edge (e0);
        \path [draw,->] (y1) edge (e0);
        \path [draw,->] (y2) edge (e0);
        \path [draw,->] (y3) edge (e0);
        \path [draw,->] (y1) edge (e1);
        \path [draw,->] (y2) edge (e1);
        \path [draw,->] (y3) edge (e1);
        \path [draw,->] (y2) edge (e2);
        \path [draw,->] (y3) edge (e2);
        \path [draw,->] (y3) edge (e3);
    
        \node[rotate=90,color=black] at (-4, 0.8) { \texttt{consistent} };
    \end{tikzpicture}
    \end{center}
        }
    \end{figure}
    
    
    
    \begin{figure}[!h]
        \floatconts
            {}
            {}
            {
    \begin{tikzpicture}
        \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=1cm] (e0) at (-3,0) {   $\sI(0)$ };
        \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=1cm] (e1) at (-1,0) {   $\sI(1)$ };
        \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=1cm] (e2) at ( 1,0) {   $\sI(2)$ };
        \node [circle,draw=black,fill=gray!20,inner sep=0pt,minimum size=1cm] (e3) at (3, 0) { $\sI(3)$ };
        \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=1cm] (y0) at (-3,1.6) { $0$ };
        \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=1cm] (y1) at (-1,1.6) { $1$ };
        \node [circle,draw=black,fill=gray!20,inner sep=0pt,minimum size=1cm] (y2) at ( 1,1.6) { $2$ };
        \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=1cm] (y3) at (3, 1.6) { $3$ };
    
        \path [draw,->] (y0) edge (e0);
        \path [draw,->] (y1) edge (e0);
        \path [draw,->] (y2) edge (e0);
        \path [draw,->] (y3) edge (e0);
        \path [draw,->] (y1) edge (e1);
        \path [draw,->] (y2) edge (e1);
        \path [draw,->] (y3) edge (e1);
        \path [draw,->] (y2) edge (e2);
        \path [draw,->] (y3) edge (e2);
        \path [draw,->] (y3) edge (e3);
    
        \node[rotate=90,color=black] at (-4, 0.8) { Incompatible };
    \end{tikzpicture}
            }
    \end{figure}
    
    
    \begin{figure}[!h]
        \floatconts
            {fig:inconsistent_tikz_example}
            {\caption{
                A graphical illustration of a case where evidence are inconsistent. Evidence are either incompatible (Top) or insufficient (Bottom). A gray node indicate existence of a positive label.
            }}
            {
    \begin{tikzpicture}
        \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=1cm] (e0) at (-3,0) {   $\sI(0)$ };
        \node [circle,draw=black,fill=gray!20,inner sep=0pt,minimum size=1cm] (e1) at (-1,0) { $\sI(1)$ };
        \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=1cm] (e2) at ( 1,0) {   $\sI(2)$ };
        \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=1cm] (e3) at (3, 0) {   $\sI(3)$ };
        \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=1cm] (y0) at (-3,1.6) { $0$ };
        \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=1cm] (y1) at (-1,1.6) { $1$ };
        \node [circle,draw=black,fill=gray!20,inner sep=0pt,minimum size=1cm] (y2) at ( 1,1.6) { $2$ };
        \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=1cm] (y3) at (3, 1.6) { $3$ };
    
        \path [draw,->] (y0) edge (e0);
        \path [draw,->] (y1) edge (e0);
        \path [draw,->] (y2) edge (e0);
        \path [draw,->] (y3) edge (e0);
        \path [draw,->] (y1) edge (e1);
        \path [draw,->] (y2) edge (e1);
        \path [draw,->] (y3) edge (e1);
        \path [draw,->] (y2) edge (e2);
        \path [draw,->] (y3) edge (e2);
        \path [draw,->] (y3) edge (e3);
    
        \node[rotate=90,color=black] at (-4, 0.8) { Insufficient };
    \end{tikzpicture}
        }
    \end{figure}
        


\begin{table}[!h]%
\floatconts
    {tab:data_split_counts}
    {\caption{Data split counts}}
    {
        \begin{tabular}{ll}
        \toprule
        \bfseries Split & \bfseries \#Images \\
        \midrule
        train    &  217016 \\
        validate &  10445  \\
        test     &  10625  \\
        \bottomrule
        \end{tabular}
    }
\end{table}
    
\begin{table}[!h]%
\floatconts
    {tab:data_split_counts}
    {\caption{Data split counts for Edema Severity}}
    {
        \begin{tabular}{ll}
        \toprule
        \bfseries Split & \bfseries \#Images \\
        \midrule
        train                         &  6656  \\
        validate                      &  648   \\
        test\_expert\_report (EP)     &  498   \\
        test\_consensus\_image (CI)   &  159   \\
        \bottomrule
        \end{tabular}
    }
\end{table}
    

